Strategies and Perceived Risks of Sending Sensitive Documents

People are frequently required to send documents, forms, or other materials containing sensitive data (e.g., personal information, medical records, financial data) to remote parties, sometimes without a formal procedure to do so securely. The specific transmission mechanisms end up relying on the knowledge and preferences of the parties involved. Through two online surveys ($n=60$ and $n=250$), we explore the various methods used to transmit sensitive documents, as well as the perceived risk and satisfaction with those methods. We find that users are more likely to recognize risk to data-at-rest after receipt (but not at the sender, namely, themselves). When not using an online portal provided by the recipient, participants primarily envision transmitting sensitive documents in person or via email, and have little experience using secure, privacy-preserving alternatives. Despite recognizing general risks, participants express high privacy satisfaction and convenience with actually experienced situations. These results suggest opportunities to design new solutions to promote securely sending sensitive materials, perhaps as new utilities within standard email workflows.

==> 99-6-revisions.tex <==
\clearpage
\section*{Major Revisions Changes}
\label{app:revisions}

We thank the reviewers for their insightful comments that have greatly improved the paper. We have made several changes based on that feedback, which we outline in this section, starting with  addressing the required changes outlined in the meta-review. Following, we outline additional changes based on individuals reviews. We have also included our \texttt{latexdiff} at the end of this document but given the sweeping nature of our changes, we suspect it will not be particularly useful.

\subsection*{Response to Meta Review}

\begin{enumerate}
\item \textit{
Providing a more thorough analysis that goes beyond the discussion of the survey quotes. This can be either:
    \begin{enumerate}
    \item A more thorough quantitative analysis, with statistical tests, to produce comparisons among the high-level categories in each research question (e.g. the scenario groups, the modes of communication, etc.). Ideally, this analysis should produce further interesting conclusions, and not only reiterate what is already in the paper.
    \item  An extension to the survey via a followup study going in-depth on the open questions that have been raised throughout. That would add new dimensions that cover more aspects of the problem space that the paper is studying.
    \end{enumerate}}    

We develop a second, follow-up survey based on the qualitative analysis found in the original survey. (The full text of \surveyTwo{} can be found in Appendix~\ref{app:survey2}.) \surveyTwo{} is predominantly closed-response, where response choices were determined from coding open-responses in \surveyOne{}. This allowed us to perform quantitative analysis that confirms and extends the findings of \surveyOne{}---namely, that participants are in general satisfied with their methods of transmitting sensitive information and usually view any potential risks as related to the actions of the \emph{recipient}, rather than the \emph{sender}.

In particular, \surveyTwo{} differs from \surveyOne{} in two important ways:
\begin{enumerate}
    \item Instead of providing \emph{scenarios} where participants indicated whether they had experienced something similar, participants were asked to identify communication \emph{methods} they had used to transmit sensitive information. Following, participants were prompted to provide a scenario when that method was used. This allows balancing of the communication methods during analysis, and also  ensures that participants are always providing responses to scenarios that are real, not imagined.
    \item Several questions were added to the survey to probe deeper into participants' satisfaction of the communication method. This includes rating the likelihood of risk, where the risk resides (with them, in transit, or at the recipient), who suggested the method, and whether they would use the method again in the same scenario.
\end{enumerate}

\item \textit{A motivation of the sample size, linking it to the expected significance of results in case of quantitative analysis. If the sample size is not justifiable, another way is to potentially extend the survey to obtain statistically significant comparisons.}

We recruited an additional 250 participants for the second survey. As part of the analysis plan, we planned a regression analysis to identify factors influencing satisfaction with a given method (Section~\ref{subsec:rq2}). Using G-power, we estimated that we can confidently identify medium effects with 200+ responses.  Additional statistical analysis, comparing overall risk (Section~\ref{subsec:rq3}), using Kruskal-Wallis test (and posthoc Mann-Whitney U-test) are also sufficiently powered with $n=250$,  and should be able to identify small effects.

\item \textit{A more extensive discussion of the design implications: how the currently available technological offerings address or fail to address the issues raised by the study.}

We have added a paragraph in the discussion about document sharing services. 
In brief, participants know they exist but do not seem to choose to use them.

\item \textit{Comparing and contrasting to the related works raised in the reviews, particularly around data deletion and data permanence.}

    We have added and emphasized work in the areas of retrospective privacy ~\cite{ruoti2017weighing,ramokapane2017feel,monson2018usability}, website authentication~\cite{sunshine2009crying,bravo2013your,schechter2007emperor}, and phishing~\cite{akhawe2013alice,petelka2019put}. We have also incorporated those findings into our discussion, emphasizing how our results confirm user assumptions that their online behavior is secure.

\end{enumerate}

\subsection*{Responses to Individual Reviews}

\paragraph{Reviewer A}
\begin{itemize}
    
    \item {\em Authors asked participants to report whether they had experienced the same or similar scenario before, however they did not ask participants to explain their experience. This makes me concerned about the real versus imagined categorization.}
    
    We agree that more details from participants about their experiences was needed. This is why in \surveyTwo{}, we asked participants to provide a scenario for a given communication method, rather than provide scenarios.
    
    \item {\em When briefing participants about the purpose of the survey, authors also mentioned that the information that is being transmitted might be sensitive. I believe mentioning the sensitivity could bias participants and as you mentioned in your related work perceptions and behaviors also depend on how sensitive the user believes the information is.}
    
    We agree that in the first survey, there is the potential for bias due to the varied perceived sensitivities of the scenarios. However, we note that prior work suggests self-reporting for security and privacy can be useful despite social desirability effects~\cite{redmiles2018asking}. We deliberately opted to include both real and hypothetical scenarios in the first survey as what participants might plan or imagine they would do in a given circumstance are still important data points. We have described this point better in the limitations section when discussing \surveyOne{}.
    
    We also designed \surveyTwo{} to have participants provide real scenarios used for a given communication method. Those findings confirm that the methods described in the first survey do match in roughly equal proportions to similar scenarios.
    
    \item {\em Since authors didn't ask participants to specify how sensitive each scenario was, I would like authors to explain how this could have impacted the study and its findings. In addition, this should also be added to the limitations section.}
    
    We agree that the perceived sensitivity of the scenario can bias the results, leading to responses that induce socially desirable responses. As noted above, we believe even these responses offer value and have been shown to be useful in security and privacy literature.
    
    In \surveyTwo{}, while we do not specifically ask about the sensitivity of a provided scenario, we ask participants to rate the associated risks they perceive in the scenario with the communication method. Overall, we find that many participants do not express high risk with any scenario, and when assigning risk, they do so at the end point or in transit, not on themselves. This aligns with the findings in \surveyOne{}.

    \item {\em The questions about satisfaction was only asked once for all the methods of communication, instead of asking participants to answer this question for all the methods. Therefore, I am not sure how to take the satisfaction findings, as it's not obvious which method they refer to. In your rebuttal, please correct me if I am wrong.}
    
    Each participant answered the satisfaction questions for each of the three scenarios they were presented, not just once. Sorry for the confusion. We have updated the description of Survey 1 in both the main body (Section~\ref{sec:methods:surveyone}) and in the appendix (Appendix~\ref{app:survey1}).

    \item {\em In the survey questions, authors said: "please note that there is no correct answer for many of these questions." Please explain why you used the word "many." Were there questions that had correct answers?}
    
    We chose this phrasing to reduce social desirability effects and encourage participants to honestly describe the method that they would use in that scenario, without imposing any judgement. We did not want participants to believe that we (as researchers) had  a "right choice" in mind that they should respond with, or feel guilt/remorse/shame for having used the wrong method. 
    
    \item {\em I am curious to know how within-participant data dependency played a role in the qualitative responses. In particular I am wondering whether authors have seen any patterns suggesting that most participants who suggested method X also suggested methods Y and Z.}
    
    When we designed \surveyTwo{}, the new focus on asking about one method meant that we were unable to answer this question. 
    However, we agree that it is an interesting question, and could be an fruitful topic for future work.
    
    \item {\em Although the recommendations in the discussion were interesting, they were not arranged well. I would suggest authors to have subsection titles by focusing on the recommendation itself.}

    We have retitled our ``Design implications'' section in the discussion section to ``Design implications and recommendations'', and added subsection titles for our specific recommendations.

    \item {\em     Please fix this sentence on page 10: One mentioned that obtaining the documents in order to send them was inconvenient. was one obstacle to successfully completing the task.}
    
    Thank you. We have fixed this typo.
    
    \item {\em Please correct this: COVID-19¿‘ [Answer: free text]}
    
    Thank you for noting this typo. It has been corrected. 

\end{itemize}

\paragraph{Reviewer B}

\begin{itemize}
    \item {\em The similarity of opinions even during social distancing was very much a surprise to me as well -- I would have thought people would have been more likely to take the risk sending things "insecurely". }
    
    We were also surprised by these findings! We still discuss COVID-19 in Section~\ref{sec:results_rq}.
    
    \item {\em One minor typo: page 9, "loosing" is written instead of "losing".}
    
    Thank you for noting this typo. It has been corrected.
\end{itemize}


\paragraph{Reviewer C}
\begin{itemize}
    \item {\em The paper seems to imply a quantitative presentation of the data, when instead they should probably stick to a qualitative analysis. In particular, no statistical analyses are performed.}
    
    In \surveyOne{}, the primary results are based on qualitative analysis, e.g., coding which communication methods were used in different scenarios or the kinds of risks involved. The quantitative analysis for \surveyOne{} is more descriptive in nature, and we agree that this is a shortcoming.
    
    To address this criticism, as part of \surveyTwo{}, we designed a primarily quantitative survey with closed responses based on the qualitative coding from \surveyOne{}. We were able to do substantially more quantitative analysis, including statistical tests and regression analysis, that provides a fuller picture of user behavior of sending sensitive documents using different methods in different scenarios. 
    
    \item {\em The qualitative analysis would benefit from further categorization within the main body. For example, what are the concepts behind why people are satisfied with convenience, or unsatisfied with convenience. The same for privacy satisfaction/dissatisfaction. The exploration presented in the paper is too shallow in my opinion. I assume there is enough data and I think a revision can present more in-depth qualitative findings.}
    
    We agree that more insight into the privacy and convenience satisfaction would improve the paper, and that the methods of \surveyOne{} do not sufficiently cover these topics. To improve the results, we designed \surveyTwo{} with additional closed-ended questions where participants specifically answer on a Likert scale their agreement with the reasons participants indicated for privacy (dis)satisfaction in \surveyOne{} and their assessment of the likelihood of certain ways their data might be mishandled, again identified from \surveyOne{} free responses.  The satisfaction responses are analyzed in a regression analysis determining which factors correlate with satisfaction. In brief, we find that compared to in person, people are less likely to be satisfied with the privacy of email, physical mail, and fax. In addition, if they are sending financial documents or there is some perception of risk at the destination, they are more likely to be dissatisfied with privacy. Participants are \emph{more} satisfied with privacy if they believe the participant will keep their data safe or if the method is inherently secure, and, perhaps unusually, if they are sending Social Security numbers.
    
    \item {\em In many cases I found the quotes to not provide enough information about the "why."}
    
    We agree that the ``why'' is missing from the responses to \surveyOne{}. We added questions to \surveyTwo{} that asked participants to indicate who suggested the method they ended up using, and if they agreed with that method (Section~\ref{sec:methods_survey_2}). 
    
    \item {\em The design implications need more work. For example, the authors say that end-to-end encryption is transparently available in WhatsApp, and then "Is something similar possible for transmitting sensitive documents? " Why can't the documents be transmitted in WhatsApp itself? This is already done. Doctors share medical records via WhatsApp in some countries.}
    
    We agree that there is no reason why WhatsApp (or Signal) could not be used for document transmission, however this does not seem to be a common practice for our US-based participants as this particular strategy was not mentioned (perhaps due to HIPPA regulations in the US). The larger point, though, about using transparently secure tools for transmitting sensitive information is a motivation for this research.
    We now also note that the US-centric aspect of our surveys in the limitations.
    
\end{itemize}

\paragraph{Reviewer D}

\begin{itemize}
    \item {\em Population was skewed young, educated, and wealthy. Since the population was recruited using Prolific, an opportunity was lost to have balanced the demographics to include more low income, elderly, etc. Comment on this in the limitations.}
    
    Related work~\cite{redmiles2016learned} indicates that demographic panels can somewhat improve demographics biases in sampling but still are not fully representative for many sub-populations. We believe that our participants provide meaningful insights despite this limitation for both \surveyOne{} and \surveyTwo{}.
    
    \item {\em No justification is given for the sample size, which is too small to generalize the results to the overall population. This should be discussed in the limitations. Perhaps the size is acceptable given the qualitative analysis. The paper seems more exploratory, providing a basis for a more detailed survey that is broadly disseminated to a more diverse sample size.}
    
    \surveyTwo{} was designed to address exactly this. Its closed-answer questions were based on the free responses from \surveyOne{} and we were able to distribute it to $n=250$ participants.
    
    \item {\em Responses could be biased because of self-reported data and participants imagining a hypothetical scenario. This should be listed as a limitation. Is there a reason the participants weren’t allowed to select three scenarios they had actually experienced? It would have the disadvantage of not balancing across the scenarios, but would have the advantage that all results are based on experience. It would be interesting to hear if/how this was part of the design process.}
    
    We note first that prior work suggests self-reporting for security and privacy can be useful despite social desirability effects~\cite{redmiles2018asking}.
    In order to address the concern about imagined scenarios, for \surveyTwo{} we asked participants to report about instances they had successfully used a given transmission method at least once.
    
    \item {\em The discussion about users not understanding data in transit and mostly being concerned about data at rest is interesting. This seems to confirm earlier work about TLS warnings and how users conflate the lock icon to refer to the site’s security posture and not the security of the data in transit. Perhaps this idea can be better-connected to prior work and emphasize it provides further confirmation.}
    
    We agree, and have added work from this area to both our related work and discussion to link it more closely with our results here.
    
    \item {\em  There are many secure document sharing services in the cloud. It would be interesting to hear a summary of these tools. Do they already address some of the design suggestions raised in the paper? In what ways do they fall short? Is the issue that we don’t have freely available tools for sharing data on the web between individual users, but businesses are more likely to have access to these kinds of tools? Some examples I found online include: docsend.com, aodocs, dropbox, box, google drive, one drive. }
    
    We agree that categorizing existing tools would be interesting, but performing a detailed analysis might be out of scope for this paper, which is more focused on the end-user experience. We have noted and discussed some of these additional options in our discussion section.
    
    \item {\em The scenario examples are US-centric. The paper refers to SSN (not explained on first usage), Social Security, Social Security Number. Consolidate/simplify usage. Page 3 - “and Social Security needed” - does that mean SSN?}
    
    Yes. That is Social Security number (SSN). We have properly introduced the acronym or used the full phrase instead. We have also noted the US-centric aspect of the surveys in the limitations.
    
    \item {\em Table 2 - the section titled “Sensitive Information” is hard to interpret until I read the actual question 8 in appendix B2. Can the title of that part be made more descriptive so the reader understands the context of those terms without relying on the question in the appendix?}
    
    We have updated the table titles to be more clear.
        
\end{itemize}
\paragraph{Reviewer E}
\begin{itemize}
    \item {\em On the other hand, the paper's depth was hindered a bit by the survey format. As the authors highlight (and I appreciate being up-front about the limitation), it is sometimes difficult to do further probing into the posed research questions. This was the case when the participants did not articulate why they were satisfied by the privacy of their chosen method.}
    
    We agree that depth was missing from \surveyOne{}, and we designed \surveyTwo{} to fill in these critical details about what leads to increased/decreased satisfaction with a method. 
    
    \item {\em The paper can benefit from highlighting the answers to the research questions throughout the sections, particularly in Section 4.}

    We have reorganized the results section by research question to describe the results for \surveyOne{} and \surveyTwo{}, and as part of that reorganization, have summarized the key findings related to each research question at the end of the relevant subsection.

    \item {\em The figures/tables in the paper are very briefly described. A lot of interesting comparisons can be drawn based on these. For example, interpreting the differences by scenario in Figure 2 or Table 4 would be interesting. There is enough unused space in the paper for such comparisons.}
    
    We agree that inter-scenario comparisons would be interesting, but we decided that due to the limitations of real vs imagined scenarios, that for \surveyTwo{} we would focus on comparison between satisfaction for transmission methods.

\end{itemize}















==> tab_demographics_2.tex <==
\begin{table}[!t]
  \centering

\caption{Survey 2 Demographics - questions are provided in Appendix~\ref{app:survey2}. The ``Sensitive Information'' question allowed participants to select multiple responses. \noel{needs education}}
\label{tab:demographics2}

\smallskip
\begin{minipage}[t]{0.4\linewidth}
    \begin{tabular}{lr}
        \multicolumn{2}{c}{\bf Identified Gender}\\ \midrule
        Female & 111 \\
        Male & 132 \\ %
        Nonbinary & 7 \\
        \\
        \multicolumn{2}{c}{\bf Age} \\ \midrule
        18-30 &  84 \\
        31-40 &  68 \\
        41-50 &  35 \\
        51-60 &  17 \\
        61+   &  10 \\
        No answer & 36 \\ %
        \\
        \multicolumn{2}{c}{\bf CS Experience}\\ \midrule
        No & 190 \\
        Yes & 54 \\
        Not sure & 2 \\
        Prefer not to say & 4 \\ \bottomrule
      \end{tabular}
    \end{minipage}
    \hspace{.2in}
      \begin{minipage}[t]{0.4\linewidth}
        \begin{tabular}{lr}
        \multicolumn{2}{c}{\bf Income Level}\\ \midrule
        < \$50,000 & 121 \\
        \$50K-\$100K & 86 \\
        > \$100K & 35 \\
          Prefer not to say & 8 \\
          \\
        \multicolumn{2}{c}{\bf Security Clearance}\\ \midrule
        No & 214 \\
        Yes & 19 \\
        Not sure & 13 \\
        Prefer not to say & 4 \\
          \\
        \multicolumn{2}{c}{\bf Sensitive Information}\\ \midrule
          Credit Card info. & 90 \\
          HIPAA Info. & 62 \\
          SSN & 85 \\
          FERPA Info. & 20 \\
          None & 111 \\ \bottomrule
        \end{tabular}
      \end{minipage}

\end{table}



==> tab_methods_first_thirty.tex <==
\begin{table*}[h]
    \centering
    \begin{tabular} {
      | >{\raggedright\arraybackslash}p{0.25\textwidth}
      | >{\raggedleft\arraybackslash}p{0.05\textwidth}
      | >{\raggedright\arraybackslash}p{0.25\textwidth}
      | >{\raggedright\arraybackslash}p{0.25\textwidth} | }
        \hline Code & Count & Description & Quote \\ \hline

        In person & 54 & Delivering the information by hand to the recipient, whether written down or simply told to them & ``I provided the information on an application in the office. It was on paper and when I was done I handed it to them'' \\ \hline

        Email & 23 & In the appendix, this category is further divided type, but is often the default answer for sending things digitally & ``I sent the password to the persons private email that I knew for a fact was only accessible by only them.'' \\ \hline

        Online form or portal & 14 & Many participants indicated that institutions (particularly banks) provided a site, app, or portal to upload these documents & ``I applied for a savings account recently, but I did it through their mobile app. Really they had all of my information, but they did ask to confirm questions like social security number and contact information.'' \\ \hline

        Direct messaging & 13 & This covers SMS, secure and insecure messaging services, and other similar modes of communication & ``I would text them the password and tell them to delete it from their phone after they are done.'' \\ \hline

        Phone call & 9 & Certain classes of information, like passwords, were communicated by phone call & ``I provided it to him over a phone call.  I do not trust electronic devices with password sending.'' \\ \hline

        Secure sending online & 6 & Some participants had a concept of  ``sending online'' but did not provide detail & ``Sending it securely online is a more convenient way to do it for everyone involved.'' \\ \hline

        Physical mail & 3 & US Postal Service, UPS, Fedex, and other services & ``I would probably print everything out and snail mail it all to the doctor.'' \\ \hline
        
        Fax & 2 & One of the rarest of cases, but still a method that is used & ``I would fax the documents to them simply because I do not trust sending that information via the internet.'' \\ \hline

        Document sharing service & 2 & Services like Google Drive, Box, or Dropbox where a document is uploaded to a shared location & ``Maybe through an app like dropbox with both password and PDF in a shareable link.'' \\ \hline


    \end{tabular}

\caption{Methods high-level codebook. Note: each participant provided methods for each of \textbf{three} scenarios, and may have provided more than one method in their response.}
\label{tab:methods}
\end{table*}


==> tab_mitigation.tex <==
\begin{table*}[!ht]
    \centering
    \begin{tabular} {
      | >{\raggedright\arraybackslash}p{0.25\textwidth}
      | >{\raggedleft\arraybackslash}p{0.05\textwidth}
      | >{\raggedright\arraybackslash}p{0.25\textwidth}
      | >{\raggedright\arraybackslash}p{0.25\textwidth} | }
        \hline \textbf{Code} & \textbf{Count} & \textbf{Description} & \textbf{Quote} \\ \hline

        Sending information digitally (generic) & 2 & Some participants were satisfied just with sending information digitally itself as a mode of mitigating risk & ``Send them digitally'' \\ \hline

        Sending information digitally (specific) & 6 & A few participants indicated specific aspects of digital security that were of note without providing a specific answer to how this would apply to the situation \noel{worth its own subtable perhaps?} & ``I could change my password afterwards'' \\ \hline

        Sending information securely (generic) & 6 & Much like when reporting methods, some participants indicated that sending information in a nonspecific secure channel was a good strategy to manage risk & ``Use only secure submissions and change my passwords often.'' \\ \hline

        Sending information securely (specific) & 10 & Some people indicated that a particular method was best - in particular, 9 of these 10 mentioned giving information in person or on paper & ``If the secure channel is still doubtful, perhaps writing a letter may provide some peace of mind.'' \\ \hline

        Keeping physical documents safe & 3 & Occasionally, keeping paper documents secure was brought up as important. & ``Bring a bag that zips, as this will make it difficult to lose documents in transportation.'' \\ \hline

        Only give information to trusted recipients & 15 & Many participants emphasized trusting the person to whom they were giving the documents & ``Verify the people I hand off to are competent and do work there.'' \\ \hline

        Ask the recipient to delete my data & 5 & Encouraging others to delete their data or delete a local copy themselves & ``Adding explicit instructions to delete the email after downloading the documents.'' \\ \hline

        Properly identify myself to the recipient & 1 & Identifying oneself to the recipient & ``Using identification as a confirmation that you are who you say you are.'' \\ \hline



    \end{tabular}

\caption{Mitigation strategies high-level codebook. This question was asked after all scenarios had been presented.}
\label{tab:mitigation}
\end{table*}


==> tab_regression_conv.tex <==
\begin{table*}[!ht]
\centering
\begin{tabular}{|l|rrrr|}
  \hline
Variable & Coefficient & Odds Ratio & P-value & Confidence Intervals \\
  \hline
HaveYouBeenNot sure & -0.15 & 0.86 & 0.92 & [0.05, 15.12] \\
  HaveYouBeenYes & 0.25 & 1.28 & 0.48 & [0.65, 2.53] \\
  Scenariotaxes & 0.47 & 1.59 & 0.48 & [0.44, 5.77] \\
  Scenariopassword & 1.36 & 3.90 & 0.05 & [1.01, 15.04] \\
  Scenarionew\_school & -0.34 & 0.71 & 0.60 & [0.2, 2.52] \\
  Scenarioapartment\_rent & 0.46 & 1.59 & 0.50 & [0.41, 6.09] \\
  ScenarioPDF & 0.56 & 1.75 & 0.40 & [0.48, 6.42] \\
  Scenariobackground\_check & -0.22 & 0.80 & 0.74 & [0.22, 2.92] \\
  Scenarionew\_checking\_account & -0.13 & 0.88 & 0.85 & [0.23, 3.32] \\
  Scenarionew\_doctor & -0.02 & 0.98 & 0.98 & [0.27, 3.55] \\
   \hline
\end{tabular}
\caption{Ordinal logistic regression - convenience satisfaction}
\label{tab:reg_conv}
\end{table*}


==> tab_regression_gen.tex <==
\begin{table*}[!ht]
\centering
\begin{tabular}{|l|rrrr|}
  \hline
Variable & Coefficient & Odds Ratio & P-value & Confidence Intervals \\
  \hline
HaveYouBeenNot sure & -1.98 & 0.14 & 0.28 & [0, 5] \\
  HaveYouBeenYes & 0.07 & 1.07 & 0.85 & [0.51, 2.26] \\
  Scenariotaxes & -0.35 & 0.70 & 0.64 & [0.16, 3.08] \\
  Scenariopassword & 0.42 & 1.53 & 0.57 & [0.35, 6.62] \\
  Scenarionew\_school & 0.35 & 1.42 & 0.64 & [0.33, 6.18] \\
  Scenarioapartment\_rent & 0.11 & 1.11 & 0.89 & [0.25, 4.93] \\
  ScenarioPDF & 0.59 & 1.80 & 0.43 & [0.42, 7.72] \\
  Scenariobackground\_check & 0.15 & 1.17 & 0.84 & [0.26, 5.17] \\
  Scenarionew\_checking\_account & 0.30 & 1.35 & 0.70 & [0.3, 6.1] \\
  Scenarionew\_doctor & 0.48 & 1.61 & 0.53 & [0.36, 7.19] \\
   \hline
\end{tabular}
\caption{Ordinal logistic regression - general satisfaction}
\label{tab:reg_gen}
\end{table*}


==> tab_regression_priv.tex <==
\begin{table*}[!ht]
\centering
\begin{tabular}{|l|rrrr|}
  \hline
Variable & Coefficient & Odds Ratio & P-value & Confidence Intervals \\
  \hline
HaveYouBeenNot sure & -1.41 & 0.24 & 0.32 & [0.01, 3.97] \\
  HaveYouBeenYes & 0.42 & 1.51 & 0.21 & [0.8, 2.88] \\
  Scenariotaxes & -0.37 & 0.69 & 0.56 & [0.21, 2.34] \\
  Scenariopassword & -0.19 & 0.83 & 0.75 & [0.25, 2.74] \\
  Scenarionew\_school & -0.23 & 0.79 & 0.70 & [0.24, 2.58] \\
  Scenarioapartment\_rent & -0.34 & 0.71 & 0.59 & [0.21, 2.43] \\
  ScenarioPDF & -0.67 & 0.51 & 0.27 & [0.16, 1.69] \\
  Scenariobackground\_check & -1.25 & 0.29 & 0.05 & [0.08, 1.01] \\
  Scenarionew\_checking\_account & -0.59 & 0.56 & 0.36 & [0.16, 1.94] \\
  Scenarionew\_doctor & -0.33 & 0.72 & 0.61 & [0.2, 2.53] \\
   \hline
\end{tabular}
\caption{Ordinal logistic regression - privacy satisfaction}
\label{tab:reg_priv}

\end{table*}


==> tab_risks.tex <==
\begin{table*}[!ht]
    \centering
    \begin{tabular} {
      | >{\raggedright\arraybackslash}p{0.25\textwidth}
      | >{\raggedleft\arraybackslash}p{0.05\textwidth}
      | >{\raggedright\arraybackslash}p{0.25\textwidth}
      | >{\raggedright\arraybackslash}p{0.25\textwidth} | }
        \hline \textbf{Code} & \textbf{Count} & \textbf{Description} & \textbf{Quote} \\ \hline
        Identity theft & 7 & Loss of personally identifiable information in order to pose as the target & ``I fear that the documents may fall into the hands of a person that would use them to to steal my identity.'' \\ \hline
        Financial harm & 2 & Loss of banking information, credit card information, or direct monetary loss  & ``The same parties mentioned in example one may also use the documents to commit other acts such as accessing my credit cards and bank information.'' \\ \hline
        Reputational damage & 0 & \noel{Do we want to indicate this was a code no-one chose? may differ with new data as well} & ``no codes yet'' \\ \hline
        Generic ``malicious'' actions & 14 & Some participants had a concept of  their data being used for ``malicious purposes'' but did not provide detail & ``Someone getting a hold of the information on your childs birth certifcate and using it maliciously'' \\ \hline
        Some institution can read the participant's emails & 1 & One participant indicated a particular threat to email specifically. & ``The other companies/organizations  who can read my emails. What will they do with that information.'' \\ \hline
        The data \textbf{in transit} is at risk & 5 & Some participants indicated a concern with the data being at risk while in transit, but were often not specific about why this was the case. & ``I am scared about losing the documents in transportation.'' \\ \hline
        The data \textbf{at rest} is at risk & 27 & A very common concern was the provenance of the data once received by the intended recipient. Many participants indicated mistrust or doubt that the recipient would use their data appropriately & ``How the place I give these documents stores or disposes of them.'' \\ \hline
        The data will be lost or misplaced & 7 & Often, participants were not concerned about the data being at risk per se, but rather the person who was supposed to have them misplacing or losing them, without a concept of further threat. & ``If I provide papers in person, it would concern me if the person loses the documents. '' \\ \hline
    \end{tabular}

\caption{Risks high-level codebook. This question was asked after all scenarios had been presented.}
\label{tab:risks}
\end{table*}


==> tab_sat_aggregate.tex <==
\begin{table*}[!ht]
    \centering
    \small
    \begin{tabulary}{\textwidth}{|L|R|R|R|R|R|R|}
        \hline

        \textbf{Scenario} &
        \textbf{Mean General Satisfaction} &
        \textbf{Mean Privacy Satisfaction} &
        \textbf{Mean Convenience Satisfaction} & \textbf{Median General Satisfaction} & \textbf{Median Privacy Satisfaction} & \textbf{Median Convenience Satisfaction} \\ \hline
        Renting an apartment & 4.05 & 4.05 & 4.20 & 4.0  & 4.0 & 4.5 \\ \hline

        Background check & 3.90 & 3.40 & 3.70 & 4.0 & 4.0  & 4.0 \\ \hline

        Applying for a mortgage & 4.10 & 4.10 & 3.80 & 4.5 & 4.0 & 4.0 \\ \hline

        Creating a new checking account & 4.15 & 3.90 & 3.85 & 4.0 & 4.0 & 4.0 \\ \hline

        Visiting a new doctor & 4.15 & 3.95 & 3.90 & 4.0 & 4.0 & 4.0  \\ \hline

        Starting a child at a new school & 4.10 & 4.05 & 3.65 & 4.0 & 4.0 & 4.0 \\ \hline

        Sharing a password to an email account & 4.30 & 4.10 & 4.60 & 4.0 & 4.0 & 5.0 \\ \hline

        Sharing a password-protected PDF & 4.05 & 3.70 & 4.05 & 4.0 & 4.0 & 4.0 \\ \hline

        Sharing financial information with a CPA & 3.85 & 3.90 & 4.15 & 4.0 & 4.0 & 4.0 \\ \hline

    \end{tabulary}
    \caption{Aggregate satisfaction statistics divided by scenario}
    \label{tab:sat_aggregate}
\end{table*}


==> tab_whysatisfied_conv.tex <==
\begin{table}[t]
  \caption{Participants reasons for being ``satisfied'' or ``very satisfied'' with the convenience of their mode of transmission.}
  \vspace{+.2in}
  \centering
    \footnotesize
\begin{tabular}{p{6cm}c}

{\bf Satisfied Convenience Response Code} & {\bf Frequency} \\
  \toprule
    My method of sending is convenient &  38 \\\midrule
    Email is convenient &  8 \\\midrule
    Direct messaging is convenient &  6 \\\midrule
    The method was neither conv. nor inconv. &  6 \\\midrule
    Delivering in person is convenient &   3 \\\midrule
    A phone call is convenient &   3 \\\midrule
    Delivering in person is inconvenient &   3 \\\midrule
    Encrypted email is convenient & 1 \\\midrule
    My method of sending is inconvenient  &   1 \\ \midrule
    I had no better option & 1 \\
   \bottomrule
\end{tabular}%
\label{tab:whysatisfied_conv}
\end{table}



==> tab_whyunsat_conv.tex <==
\begin{table}[t]
  \caption{Participants reasons for being ``unsatisfied'' or ``very unsatisfied'' with the convenience of their mode of transmission.}
\label{tab:whyunsat_conv}
\centering
\vspace{+.2in}
  \footnotesize
\begin{tabular}{p{6cm}c}
{\bf Unsatisfied Convenience Response Code} & {\bf Frequency} \\
  \toprule
    Delivering the documents in person is inconvenient &  5 \\\midrule
    The method was inconvenient (no fur. spec.) &   4 \\\midrule
    Gathering the required information is inconvenient &   3 \\\midrule
    Faxing the information is inconvenient & 2 \\\midrule
    The method was neither conv. or inconv. &   2 \\\midrule
    The method was convenient &   1 \\\midrule
   \bottomrule
\end{tabular}
\end{table}



==> tab_whyunsat_priv.tex <==
\begin{table}[t]
  \caption{Participants' reasons for being ``unsatisfied'' or ``very unsatisfied'' with the privacy of their mode of transmission.
  Participant answers may have contained more than one code.}
\label{tab:whyunsat_priv}
\centering
\vspace{+.2in}
\begin{tabular}{p{6.2cm}r}
\toprule
{\bf Unsatisfied Privacy Response Code} & {\bf Frequency} \\
  \midrule
    My method of sending is insecure &  12 \\
    I am unsatisfied (no specification) &   6 \\
    My method of sending is secure &   3 \\
    The recipient may unintentionally disclose  &   3 \\
    I have a COVID-related concern &   2 \\
    The recipient will intentionally disclose &   2 \\
    The recipient will keep my information safe &   1 \\
    I am unsure about the security of my method &   1 \\
   \bottomrule
\end{tabular}
\end{table}


